CoRMF: Criticality-Ordered Recurrent Mean Field Ising Solver

We propose an RNN-based efficient Ising model solver, the Criticality-ordered Recurrent Mean Field (CoRMF), for forward Ising problems. In its core, a criticality-ordered spin sequence of an $N$-spin Ising model is introduced by sorting mission-critical edges with greedy algorithm, such that an autoregressive mean-field factorization can be utilized and optimized with Recurrent Neural Networks (RNNs). Our method has two notable characteristics: (i) by leveraging the approximated tree structure of the underlying Ising graph, the newly-obtained criticality order enables the unification between variational mean-field and RNN, allowing the generally intractable Ising model to be efficiently probed with probabilistic inference; (ii) it is well-modulized, model-independent while at the same time expressive enough, and hence fully applicable to any forward Ising inference problems with minimal effort. Computationally, by using a variance-reduced Monte Carlo gradient estimator, CoRFM solves the Ising problems in a self-train fashion without data/evidence, and the inference tasks can be executed by directly sampling from RNN. Theoretically, we establish a provably tighter error bound than naive mean-field by using the matrix cut decomposition machineries. Numerically, we demonstrate the utility of this framework on a series of Ising datasets.

==> boarder.tex <==
The deliverables of the proposed research include easy-to-use software packages, which directly help scientists to explore and analyze complex combinatorial statistical systems.


==> notation.tex <==
\section*{Notations and Conventions}
To be filled.


==> old_theory_sec.tex <==

\subsection{Preliminaries}


Following the \cite{frieze1999quick,jain2018mean, jain2017approximating}'s notation, we index the rows and columns of any $m\times n$ matrix $M$ by sets $[m]$ and $[n]$, where $[k]=\{1,\cdots,k\}$ denotes a set of numbers up to $\abs{[k]}=k$.

 

\paragraph{Naive Mean-Field.}
We first derive an useful expression of the naive mean-field ansatz $Q_\theta(\bX)=\prod_{i=1}^{N} q_{i,\theta}(\bx_i)$ for later convention.
Starting from the variational mean-field free energy
\bea
\calF_{\theta}=
\E_{Q_\theta}\[E(\bX) + \frac{1}{\beta}\ln Q_{\theta}(\bX)\],\label{free_energy}
\eea 
by denoting $q_{i,\theta}(+1)\coloneqq p_{i,\theta}$ and 
$q_{i,\theta}(-1)\coloneqq1-p_{i,\theta}$, the first term on the RHS gives
\bea
\E_{Q_\theta}\[E(\bX)\]&=& \E_{Q_\theta}\(\sum_{ij}J_{ij}\bx_i\bx_j+\sum_i h_i\bx_i\)
=\sum_{ij}J_{ij}\;\E_{q_{i,\theta}} (\bx_i)\E_{q_{j,\theta}} (\bx_j)+\sum_i h_i \;\E_{q_{i,\theta}} (\bx_i) \nonumber \\
& =& \sum_{ij}J_{ij}\(2p_{i,\theta}-1\)\(2p_{j,\theta}-1\)+\sum_i h_i (2p_{i,\theta}-1).
\eea 
As for the second term, recalling the entropy $H(\cdot)\coloneqq - \sum P(\cdot)\ln P(\cdot)$ , we have
\bea
\E_{Q_\theta}\[\ln Q_{\theta}(\bX)\]=\sum_i \E_{q_{i,\theta}} \[\ln q(\bx_i)\]
=\sum_i p_{i,\theta} \ln p_{i,\theta}-(1-p_{i,\theta})
\ln p_{i,\theta}
=-\sum_i H\(p_{i,\theta}\).
\eea
Thus, we can rewrite the variational free energy of naive mean-field as
\bea
\calF_{\theta,\text{naive}}(\bar{x}_1,\bar{x}_2,\cdots,\bar{x}_n)=
 \sum_{ij}J_{ij}\bar{x}_i\bar{x}_j+\sum_i h_i \bar{x}_i-\frac{1}{\beta}\sum_i H\(\frac{\bar{x}_i+1}{2}\),
\eea 
by associating the mean-field value of the $i$th spin with $p_{i,\theta}$ via
$(2p_{i,\theta}-1)\equiv \bar{x}_i \in [-1,1].$ 
Therefore, the minimization of the variational free energy of naive mean-field becomes the following peculiar form for later conventions:
\bea 
\label{eqn:naive_MF}
\boxed{
\calF^\star_{\text{naive}}
\coloneqq
\calF_{\theta^\star,\text{naive}}
=\underset{ \bar{X}\in [-1,1]^N}{\Min}
\left[ 
\(\sum_{ij} J_{ij}\bar{x}_i\bar{x}_j+\sum_i h_i \bar{x}_i\)
-\frac{1}{\beta}\sum_i H\(\frac{\bar{x}_i+1}{2}\) \right ],
}
\eea 
where the optimized mean-field values of $\calF^\star_{\text{naive}}$, $\bar{X}^\star\coloneqq \{\bar{x}_1^\star,\cdots,\bar{x}_N^\star\}$, are associated with the optimized variational parameters $\theta^\star$.
From a graphical perspective, the naive mean-field ansatz eliminates all edges between nodes, and \eqref{eqn:naive_MF} gives an intuitive grasp of how the entropy term is involved in the optimal free energy according to the conventional $\calF = E -TS$ convention. (see Sec.~\ref{sec:F_phyiscs}). 



\paragraph{External Field Absorption.}
For the simplicity of the main proof, we provide the following lemma to convert any Ising model into its non-external-field formulation. 
\begin{claim}
\begin{lemma}[External Field Absorption]
\label{lemma:equivalent}
For any Ising model $\calG=(V,E)$ of $N$ binary spins ($\bx_i=\{\pm1\}$) with non-zero external field $h$, $\calG$ can be represented as another \textit{extended} Ising model $\Tilde{\calG}$ of $(N+1)$ spins without external field by adding one auxiliary binary spin variable $\bx_{N+1}=\{\pm1\}$ connected to every node of the graph $\calG$. 
If strength matrices and external fields of the two models are then linked via the following relation
\bea
\tilde{J}_{ij}=
    \begin{cases}
        h_i, & \text{for } j=N+1\\
        0,  & \text{for } i=N+1\\
        J_{ij}, & \text{else }\label{lemma_equi}
    \end{cases}
\eea
where $\tilde{J}$ is a $(N+1)\times (N+1)$ \textit{asymmetric} matrix with $h$ as its last column and zeros as its last row, the free energies of the two Ising models are equivalent up to an additive constant.
\end{lemma}
\end{claim}
\begin{proof}[Proof of Lemma~\ref{lemma:equivalent}]
We first write down the energy function of $\tilde{\calG}$ by adding an auxiliary spin $\bx_{N+1}=\{\pm1\}$ to $\calG$ following \eqref{lemma_equi}:
\begin{align}
\tilde{E}(\bX,\bx_{N+1})
=\sum_{i,j=1}^{N+1} \tilde{J}_{ij}\bx_i\bx_j 
=\sum_{i,j=1}^{N}J_{ij}\bx_i\bx_j+\(\sum_{i=1}^{N} h_i\bx_i\)\bx_{N+1}.
\end{align}
On the basis of which, the corresponding partition function can be expressed as
\begin{align}
\tilde{\calZ}&=\sum_{\bX; \bx_{N+1}\in \{\pm1\} } \exp{-\beta \tilde{E}(\bX)}  \\
& =\sum_{\bX} \exp{-\beta \(\sum_{i,j=1}^{N}J_{ij}\bx_i\bx_j+\sum_{i=1}^{N} h_i\bx_i\)}+\sum_{\bX} \exp{-\beta \(\sum_{i,j=1}^{N}J_{ij}\bx_i\bx_j-\sum_{i=1}^{N} h_i\bx_i\)} \nonumber \\
& = 2 \sumX \exp{-\beta \(\sum_{i,j=1}^{N}J_{ij}\bx_i\bx_j+\sum_{i=1}^{N} h_i\bx_i\)}
=2 \calZ, \annot{(Ising Parity Symmetry)}
\end{align}
indicating the free energies $\calF=-\ln \calZ / \beta$ of the two Ising models are equivalent up to an additive logarithmic-constant.
\end{proof}
\begin{corollary}\label{coro:ext_J_h}
Following Lemma~\ref{lemma:equivalent}, we have
$\norm{\tilde{J}}^2_{F}=\|J\|^2_{F}+\|h\|^2_{F}.$ 
\end{corollary}
\begin{proof}[Proof of Corollary~\ref{coro:ext_J_h}.]
Corollary~\ref{coro:ext_J_h} is an immediate result of \eqref{lemma_equi}.
\end{proof}
\begin{remark}
With Lemma~\ref{lemma:equivalent}, we now ready to apply results of matrix cut decomposition \cite{jain2018mean,frieze1999quick} to prove our error bound.
For the ease of notation, from now on we denote $N+1=N$ and $\beta=1$ without loss of generality by keeping in mind that we are always working with Ising models without external fields\footnote{Namely, we can cast any Ising model with external field into another Ising model with the same $\calF$ but with no external field.}.
\end{remark}



\begin{claim}
\begin{lemma}[Trivial Bound for Naive Mean-Field]
\label{lemma:trivial_bound_naiveMF}
Following \eqref{eqn:naive_MF}, we have the following trivial bound
\bea
\calF^\star_{\text{naive}}-\mathcal{F} \le N \norm{J}_F,
\eea
for naive mean-field.
\end{lemma}
\end{claim}
\begin{proof}[Proof of Lemma~\ref{lemma:trivial_bound_naiveMF}]
According to \eqref{eqn:naive_MF}, we have 
$\calF^\star_{\text{naive}} \leq -N \ln2.$ 
As for $\calF$, we have
\bea
\calF=-\ln (\sum_{\bX}\exp{-\sum_{ij}J_{ij}\bx_{i}\bx_{j}}) \geq -\ln \(2^N \exp{N \norm{J}_F}\)
=-N\ln2-N\norm{J}_F.
\eea
Therefore we arrive the trivial bound
$\calF^\star_{\text{naive}}-\mathcal{F} \le N \norm{J}_F.$
\end{proof}


\paragraph{Bound for Generalized Mean-Field.}
Given the fact that RNN is able to learn the independent product distribution (given the special case of the population distribution can be completely factorized into independent form), we have the next Lemma
\begin{claim}
\begin{lemma}
\label{lemma:F_RNN}
Any generalized mean-field $\calF_{\text{general}}$, that includes the naive mean-field as a member of its model family, has the following property
: $\abs{\mathcal{F}^\star_{\text{naive}}-\calF} \geq \abs{\calF^\star_{\text{general}}-\calF}.$

\end{lemma}
\end{claim}


\begin{remark}
Lemma~\ref{lemma:F_RNN} states that as the \red{naive mean field} belongs to the family of autoregressively factorized distributions, we have 
$\abs{\mathcal{F}^\star_{\text{naive}}-\calF} \geq \abs{\calF^\star_{\text{RNN}}-\calF}.$
\end{remark}



\subsubsection{Matrix Cut Decomposition Machinaries}

\begin{claim}
\begin{definition}[Cut Matrix]
Given the column subset $[s]\subseteq[m]$, the row subset $[t]\subseteq [n]$ and a real value $d$, we define the $[m]\times [n]$ \textit{Cut Matrix} $\mathsf{CUT}([s],[t],d)$ by
\bea
\mathsf{CUT}_{ij}([s],[t],d) = 
\begin{cases}
    d\quad \text{if } (i,j)\in [s]\times [t],\\
    0\quad \text{otherwise}.
\end{cases}
\eea
\end{definition}
\begin{definition}[Cut Decomposition]
The width-$p$ \textit{Cut Decomposition} of a give matrix $A$ is defined by
\bea
A = D^{(1)} + D^{(2)} + \cdots +D^{(p)} + W,
\eea
where $D^{(\mu)} \coloneqq \mathsf{CUT}\([s]_\mu,[t]_\mu,d_\mu\) $ for $\mu=1,\cdots, p$.
We say such a decomposition has \textit{width} $p$, \textit{coefficient length} $\(\sum_{\mu=1}^p d_\mu^2\)^{\nicefrac{1}{2}}$ and \textit{error} $\norm{W}_C$.

\end{definition}

\end{claim}
With these definitions, we introduce the following matrix norms:
\bea
\norm{M}_F &\coloneqq& \sqrt{\sum_{(i,j)\in [m]\times [n]} M_{ij}^2},\quad (\text{Forbenius Norm})\\
\norm{M}_{\infty} &\coloneqq&
\underset{(i,j)\in [m]\times [n]}{\Max} \abs{M_{ij}},\quad  (\text{Maximum Norm})\\
\norm{M}_C &\coloneqq& \underset{[s]\subseteq[m],[t]\subseteq [n]}{\Max} \abs{M\([s],[t]\)},\quad  (\text{Cut Norm})\\
\|W\|_{\infty \mapsto 1} &\coloneqq& \underset{\|\bX\|_{\infty}\leq 1}{\Max}\|W\bX\|_{1},\quad (\text{Infinity-to-One Norm})
\eea
where $M\([s],[t]\)\coloneqq \sum_{(i,j)\in [s]\times [t]}M_{ij}$ and
$\|W\bX\|_{1}\coloneqq \sum_i\abs{\sum_j W_{ij}\bx_j}$.




















\begin{claim}
\begin{lemma}[Cut Perturbation \cite{frieze1999quick,jain2018mean}]\label{lemma:E_decomposed_bound}
Following above definitions of $J, D^{1},\dots,D^{p}$, given real numbers $s_{\mu},s'_{\mu},t_{\mu},t'_{\mu}$ for each $\mu\in[p]$ and some 
$\gamma \in (0,1)$ such that $\abs{s_\mu},\abs{t_\mu},\abs{s'_\mu},\abs{t'_\mu} \le N$, 
$\abs{s_\mu - s'_\mu} \le \gamma N$ and $\abs{t_\mu - t'_\mu} \le \gamma N$ 
for all $\mu\in[p]$, we have
$-8\norm{J}_F\gamma N \sqrt{p}\le \sum_\mu d_\mu
\abs{r'_\mu c'_\mu - r_\mu c_\mu} \le 8\norm{J}_F\gamma N \sqrt{p}$. 
\end{lemma}
\end{claim}
\begin{proof}[Proof of Lemma~\ref{lemma:E_decomposed_bound}]
Using the argument of \cite[Lemma~19]{jain2018mean},
since $$ \abs{s'_\mu t'_\mu - s_\mu t_\mu} \le \abs{t'_\mu||s'_\mu - s_\mu} + \abs{t_\mu}\abs{s'_\mu - s_\mu} \le 2\gamma N^2,$$
we have
\begin{align*}
\(\sum_{\mu=1}^p d_\mu\abs{s'_\mu t'_\mu - s_\mu t_\mu}\)^2
&\le \(\sqrt{p}\cdot \sqrt{\sum_\mu^p d_\mu^2}\cdot  2\gamma N^2\)^2 \annot{(By Cauchy-Schwartz inequality)}
\\
&\le \(8\sqrt{p}\norm{J}_F\gamma N \)^2,
\annot{($\sqrt{\sum_\mu^p d_\mu^2}\le 4\norm{J}_F/N$ from Lemma~\ref{lemma:Frieze_Kannan})}
\end{align*} 
which implies
$-8\norm{J}_F\gamma N \sqrt{p}\le \sum_\mu d_\mu
\abs{r'_\mu c'_\mu - r_\mu c_\mu} \le 8\norm{J}_F\gamma N \sqrt{p}$.
\end{proof}
\begin{corollary}
\label{coro:dst_parity}
Lemma~\ref{lemma:E_decomposed_bound} is invariant under the transformation $d_\mu\leftrightarrow -d_\mu$, namely
$-8\norm{J}_F\gamma N \sqrt{p}\le \sum_\mu -d_\mu
\abs{r'_\mu c'_\mu - r_\mu c_\mu} \le 8\norm{J}_F\gamma N \sqrt{p}$ is also true.
\end{corollary}
\begin{proof}[Proof of Corollary~\ref{coro:dst_parity}.]
Omitted.
\end{proof}
\begin{corollary}
\label{coro:exp_dst}
Since $
\exp{\sum_{\mu=1}^p -d_\mu  {s_\mu t_\mu}}
\leq 
\exp{\sum_{\mu=1}^p -d_\mu  {s'_\mu t'_\mu}}
\exp{8\sqrt{p}\norm{J}_F\gamma N}
$,
we can simply have
$
\exp{\sum_{\mu=1}^p -d_\mu  {s_\mu t_\mu}}
\leq
 \exp{8\sqrt{p}\norm{J}_F\gamma N}
\exp{-\sum_{\mu=1}^p d_\mu  {s'_\mu t'_\mu}}
$.
\end{corollary}
\begin{proof}[Proof of Corollary~\ref{coro:exp_dst}.]
A detailed proof is shown in the supplementary materials, see  Sec.~\ref{appendix:coro_exp_dst}.
\end{proof}






\begin{claim}
\begin{lemma}[\cite{jain2018mean}]
\label{thm:naive_MF_bound} 
Let $J$ and $D$ be the matrices of interaction strengths and vectors of external fields of 
Ising models with partition functions $\calZ_{J}$ and $\calZ_{D}$, and variational free energies $\mathcal{F}_{J,\text{naive}}$ and $\mathcal{F}_{D,\text{naive}}$ of naive mean-field. 
Then, with $W:= J - D$, 
we have  
\bea
\left|\ln \calZ_J-\ln \calZ_{D}\right|\leq \abs{W}_{\infty \mapsto 1},
\eea
and 
\bea
\left|\mathcal{F}^\star_{J,\text{naive}}-\mathcal{F}^\star_{D,\text{naive}}\right|\leq\|W\|_{\infty \mapsto 1}.
\eea
\end{lemma}
\end{claim}
\begin{proof}[Proof of Lemma~\ref{thm:naive_MF_bound}]
\cite[Lemma~17]{jain2018mean} provides the original proof and we restate it here only for self-containedness.
For any spin configuration $\bX\in\{\pm1\}^{N}$, we have 
\begin{align}
\abs{E_J(\bX) -E_D(\bX)}
&=\left|\(\sum_{i,j}J_{ij}\bx_i\bx_j\)-\(\sum_{i,j}D_{ij}\bx_i\bx_j\)\right| \\
&\leq
\left|\sum_{i}\(\sum_{j}W_{ij}\bx_j\)\bx_i\right| \annot{(\text{Cauchy-Schwartz inequality)}}\nonumber\\
& \leq 
\left|\sum_{i}\(\sum_{j}W_{ij}\bx_j\)\right| \leq\|W\|_{\infty\mapsto1},
\end{align}
which implies
\begin{equation}
\exp(-\sum_{i,j}J_{ij}\bx_i\bx_j) \in \left[ \exp\left(-\sum_{i,j}D_{ij}\bx_i\bx_j \pm \|W\|_{\infty \mapsto 1} \) \right],
\end{equation}
and 
\red{
$\left|\mathcal{F}^\star_{J,\text{naive}}-\mathcal{F}^\star_{D,\text{naive}}\right|
\leq\|W\|_{\infty \mapsto 1}$ 
}
according to \eqref{eqn:naive_MF}.
Taking the sum over all configurations
and take the logarithm on both sides, we arrive 
\bea
\ln\calZ_J=\ln\[\sumX \exp(-\sum_{i,j}J_{ij}\bx_i\bx_j) \]
\in
\ln \left[ \sumX \exp\left(-\sum_{i,j}D_{ij}\bx_i\bx_j \)  \right]\pm \|W\|_{\infty \mapsto 1},
\eea
which implies $\abs{\ln\calZ_J-\ln \calZ_D}\le \|W\|_{\infty \mapsto 1}$.
An extension of this theorem with external fields is provided in Sec.~\ref{thm:naive_MF_bound_with_h}.
 
\end{proof}
\begin{remark}
For the ease of notation, we use the shorthand $\calF^\star_J=\mathcal{F}^\star_{J,\text{naive}}$ and $\calF^\star_D=\mathcal{F}^\star_{D,\text{naive}}$ in the following sections.
\end{remark}


\subsection{Main Theorem}
Now we can sate our main result --- a provably error bound for CoRMF.
\begin{claim}
\begin{theorem}[Main Theorem]
\label{thm:main_thm}
Given an Ising model $J$ of $N$ nodes and its free energy $\calF$, the CoRMF approximates $\calF$ with $Q_\theta$ following the error bound
\bea
 \frac{1}{\beta}\textsf{KL}\(Q_{\theta}|P\)
=
\mathcal{F}^\star_{\text{CoRMF}}- \mathcal{F}
\le 42 N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}\(48 N \norm{J}_F + e\),
\eea
which is equivalent to a lower bound of the KL-divergence \eqref{eqn:KL}.
\end{theorem}
\end{claim}


\begin{claim}
\paragraph{Proof Sketch.} 
Since NN gives only inaccessible black-box functions, it is hard to compute the error bound $\calF_{\text{RNN}}^\star-\calF$ for CoRMF directly.
To circumvent, we first construct the naive mean-field error bound
$\calF_{\text{naive}}^\star-\calF$, and then treat it as an inclusive special example of CoRMF (Lemma~\ref{lemma:F_RNN}) to obtain  $\calF_{\text{RNN}}^\star-\calF \le
        \calF^\star_{\text{naive}}-\mathcal{F}$
as the error bound for CoRMF.

In order to obtain $\calF^\star_{J,\text{RNN}}-\mathcal{F}$,
    we first provide the naive mean-field error bound
    $\calF^\star_{J,\text{naive}}-\mathcal{F}$ by 
    dividing it into three terms
        \bea
        \calF^\star_{J,\text{naive}}-\mathcal{F}
        \leq 
        \blue{|\ln \calZ -\ln \calZ_{D}|}
        +
        \Blue{|\calF^\star_{J,\text{naive}}-\mathcal{F}^\star_{D,\text{naive}}|
        }
        +
        \green{|\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}|},\label{ineq_3terms}
        \eea
    control them separately, and finalize the proof by using Lemma~\ref{lemma:F_RNN}.
    \begin{itemize}\setlength\itemsep{0em}
        \item \textbf{Step 1:}
        To control \blue{$|\ln \calZ -\ln \calZ_{D}|$}, $\Blue{ |\calF^\star_{J,\text{naive}}-\mathcal{F}^\star_{D,\text{naive}}|}$,
        we use cut decomposition to find suitable $D$ and apply Lemma~\ref{thm:naive_MF_bound}.
        
        \item \textbf{Step 2:}
        To control \green{$|\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}|$}, we introduce another $\gamma$-parametrized variational ansatz $\ln \calZ_{D,\gamma}^\star$ 
        such that
        \bea
        \green{
        \abs{\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}}
        }
        \le 
        \abs{\ln \calZ_{D}- 
        \ln \calZ_{D,\gamma}^\star}
        +
        \abs{\ln \calZ_{D,\gamma}^\star-\mathcal{F}^\star_{D,\text{naive}}},
        \eea
        where $|\ln \calZ_{D}- 
        \ln \calZ_{D,\gamma}^\star|$ and $|\ln \calZ_{D,\gamma}^\star-\mathcal{F}^\star_{D,\text{naive}}|$ can be controlled  by using cut perturbation Lemma~\ref{lemma:E_decomposed_bound}.
    
        \item \textbf{Step 3:}
        Combining above, we arrive the bound for $|\calF^\star_{J,\text{naive}}-\mathcal{F}|$ as follows: 
        \bea
        &\calF^\star_{J,\text{naive}}-\mathcal{F} \leq 
        \blue{
        \abs{\ln \calZ -\ln \calZ_{D}}
        }
        +
        \Blue{\abs{\calF^\star_{J,\text{naive}}-\mathcal{F}^\star_{D}}
        }
        +
        \green{\abs{\ln \calZ_{D}- 
        \ln \calZ_{D,\gamma}^\star}+\abs{\ln \calZ_{D,\gamma}^\star+\mathcal{F}^\star_D}.
        }\nonumber
        \eea
        
        \item \textbf{Step 4:}
        The bound for $\calF_{J,\text{CoRMF}}^\star-\calF$ can be obtain via Lemma~\ref{lemma:F_RNN}:
        \bea
        \calF_{J,\text{CoRMF}}^\star-\calF\le
        \calF^\star_{J,\text{naive}}-\mathcal{F}
        \le 42 N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}\(48 N \norm{J}_F + e\).
    \eea
        
    \end{itemize}
    

\end{claim}






\subsection{Main Proof}


\begin{proof}[Proof of Theorem~\ref{thm:main_thm}]
Here we quickly review the proof \cite{jain2018mean} and provide the omitted proof of their paper by including the external field.

\paragraph{Error Bound for Naive Mean-Field with External Field.}
We now claim that one can derive the simple bound with external field using \cite{jain2018mean}.

\subsubsection{Step 1: Controlling $\abs{\ln \calZ_J -\ln \calZ_{D}}$ and $\abs{\mathcal{F}^\star_J-\mathcal{F}^\star_{D}}$}

We define the cut-decomposed matrix as  $D:=D^{(1)}+\dots+D^{(p)}$, where $D^{(1)},\cdots,D^{(p)}$ are the cut matrices coming from $J$ according to Lemma~\ref{lemma:Frieze_Kannan} with the particular parameter choice $\epsilon\to\epsilon/12$ (i.e. $16/\epsilon^2\to 2304/\epsilon^2$), so that $p \le 2304/\epsilon^2$ and 
$$\norm{W}_{\infty\mapsto1}
=\|J - D\|_{\infty \mapsto 1} 
\leq \frac{\epsilon}{3} N\norm{J}_F.
$$ 
By Theorem.~\ref{thm:naive_MF_bound}, it follows that 
\bea
\boxed{
\blue{\abs{\ln \calZ_J -\ln \calZ_{D}}\leq \frac{\epsilon}{3} N\norm{J}_F}, \quad \text{and} \quad
\Blue{\abs{\calF^\star_{J}-\mathcal{F}^\star_{D}}\leq \frac{\epsilon}{3} N\norm{J}_F }.
}
\label{eqn:bound1&2}
\eea




\subsubsection{Step 2: Controlling $\abs{\ln \calZ_{D}-
\ln \calZ_{D,\gamma}^\star}$ and $\abs{\ln \calZ_{D,\gamma}^\star + \mathcal{F}^\star_D }$}

\begin{claim}
What's left is to control $|\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}|$ by using Lemma~\ref{lemma:E_decomposed_bound} and introducing another $\gamma$-parametrized variational ansatz $\ln \calZ_{D,\gamma}^\star$ to control
    $|\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star|$ and $|\ln \calZ_{D,\gamma}^\star-\mathcal{F}^\star_{D,\text{naive}}|$ such that the inequality
    \bea
    \abs{\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}}
    \le 
    \abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}
    +
    \abs{\ln \calZ_{D,\gamma}^\star-\mathcal{F}^\star_{D,\text{naive}}},\label{ineq_cool}
    \eea
    bounds $|\ln \calZ_D - \mathcal{F}^\star_{D,\text{naive}}|$. 
    In the following, we first derive the bounds for $\abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}$ and $\abs{\ln \calZ_{D,\gamma}^\star-\mathcal{F}^\star_{D,\text{naive}}}$ in \textbf{Step 2}, and finalize the proof by combining these results in \textbf{Step 3}.
\end{claim}
We first explicitly write down the partition function of the \textit{cut-decomposed matrix} $D$
\bea
\calZ_{D}=
\sumX \exp{ -\sum_{\mu=1}^p \(\sum_{i\in [s]_\mu, j\in [t]_\mu} D_{ij}^{(\mu)} \bx_i\bx_j\)}
=
\sumX\exp{-\sum_{\mu=1}^{p}S_{\mu}(\bX)T_{\mu}(\bX)d_{\mu}},
\eea
with the shorthand notation $S_{\mu}(\bX)\coloneqq \sum_{i\in [s]_{\mu}}\bx_{i}\in \[-\abs{s_\mu},\abs{s_\mu}\]$ and $T_{\mu}(\bX)\coloneqq \sum_{j\in [t]_{\mu}}\bx_{j}\in \[-\abs{t_\mu},\abs{t_\mu}\]$.
By denoting $\Vec{S}(\bX)\coloneqq\(S_{1}(\bX),\cdots,S_{p}(\bX)\)$ the vector ranges over all elements of $\[-|s_{1}|,|s_{1}|\]\times\dots\times\[-|s_{p}|,|s_{p}|\]$ for each configuration $\bX$
(and similarly for $\Vec{T}(\bX)$), and replacing $\sumX$ with the sum over all possible $\vec{S}(\bX)$'s
and $\vec{T}(\bX)$'s realizations $\sum_{\Vec{S},\Vec{T}}$
, we obtain the inner-product representation for $\calZ_D$:
\bea
\label{eqn:Z_D_innerproduct}
\calZ_{D}
=\sum_{\Vec{S},\Vec{T}}\exp\left(-\sum_{\mu=1}^{p}S_{\mu}T_{\mu}d_{\mu}\right)\left(\sum_{\{\bX:\Vec{S}(\bX)=\Vec{S},\Vec{T}(\bX)=\Vec{T}\}}1\),
\eea
where $\sum_{\mu=1}^{p}S_{\mu}T_{\mu}d_{\mu}\coloneqq \bra{S_{\mu}}d_\mu\ket{T_{\mu}}$ denotes the $d_\mu$-weighted inner product between $\vec{S}$ and $\vec{T}$.



In order to apply Lemma~\ref{lemma:E_decomposed_bound} and construct a bound for $\abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}$, we do the follows:
\begin{claim}[Construct Variational Ansatz Proof Sketch]
\begin{itemize}
    \item Given a cut-decomposition $D$, we can map the configurations $\{\bX\}$ onto the $\vec{S}$-$\vec{T}$ plane.
    
    \item
    For each point in $\vec{S}-\vec{T}$ plane, we define the corresponding local configuration set $\calX_{\Vec{S},\Vec{T},\gamma}$.
    
    \item 
    We discretize $\vec{S}$-$\vec{T}$ with hyper-grid of size $\gamma N$,
    and use $\calX_{\Vec{S},\Vec{T},\gamma}$ to expand a hypercube of size $2\gamma N$ at each realization $(\vec{S},\vec{T})$.


    \item 
    \red{
    We define $\calZ_{D,\gamma}^\star$ as the optimal term approximation to $\calZ_D^\star$ for given $\gamma$ capturing the $\vec{S}$-$\vec{T}$ point that contributes the most.
    }
\end{itemize}
\end{claim}
For any realization $\Vec{S} \in [-|s_1|,|s_1|]\times\dots\times[-|s_p|,|s_p|]$, $\Vec{T} \in [-|t_1|,|t_1|]\times\dots\times[-|t_p|,|t_p|]$ and the  $\gamma \in (0,1)$, 
we define the \textit{local configuration set} centered at $(\vec{S},\vec{T})$ with grid size $2\gamma N$ as 
\bea
\calX_{\Vec{S},\Vec{T},\gamma}
\coloneqq 
\big\{\bX\in \{\pm1\}^{N}: |S_\mu(\bX)-S_\mu| \leq \gamma N, |T_\mu(\bX)-T_\mu| \leq \gamma N \text{ for all } \mu \in [p]\big\},
\label{eqn:local_set}
\eea
such that 
$\(\vec{S}(\bX),\vec{T}(\bX)\)\big|_{\bX\in \calX_{\Vec{S},\Vec{T},\gamma}}$ 
denotes realizations close to $(\vec{S},\vec{T})$ within error $\gamma N$. 


With $\calX_{\Vec{S},\Vec{T},\gamma}$, we further introduce the \textit{auxiliary hyper-grid} 
$I_\gamma \coloneqq \{\pm\gamma N, \pm 3\gamma N,\pm 5\gamma N,\cdots,\pm\ell \gamma N\}$ to fine-grain $\vec{S}$-$\vec{T}$ 
space with an auxiliary  $\vec{S}_\gamma $-$ \vec{T}_\gamma$ space, where $\ell$ is defined to be the smallest odd integer satisfying 
$\abs{\ell \gamma N - N} \leq \gamma N$
in order to completely capture all configurations in $\vec{S}$-$\vec{T}$ space, so that $\abs{\ell}\le 1/\gamma +1$ and $\abs{I_{\gamma}} \le 1/\gamma + 2$. 
In the auxiliary fine-grained $\vec{S}_\gamma $-$ \vec{T}_\gamma$ space, we define the following $\gamma$-parametrized lower bound of the optimal partition function of $D$, i.e. $\calZ_D^\star$ (the optimal value of $\calZ_D$ in $\vec{S}$-$\vec{T}$ space):
\bea
\label{eqn:Z_D_variational}
\calZ_{D,\gamma}^\star
\coloneqq
\max_{\vec{S}_\gamma,\vec{T}_\gamma\in I_{\gamma}^{p}}\exp\(-\sum_{\mu=1}^{p}S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)}d_{\mu}\)
\bigg(\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}}\bigg)
,
\eea
where 
$\vec{S}_\gamma \coloneqq
(S_1^{(\gamma)},\cdots, S_p^{(\gamma)})$, 
$\vec{T}_\gamma \coloneqq (T_1^{(\gamma)},\cdots, T_p^{(\gamma)})$, $I_\gamma^p \coloneqq \overbrace{I_\gamma \times \cdots \times I_\gamma}^{p}$, and $|\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}|$ 
counts the number of configurations captured by the local configuration set centered at $(\vec{S}_\gamma,\vec{T}_\gamma)$, see 
Figure~\ref{fig:1}.
Intuitively, we should first note that, if we take the continuous limit $\gamma \to 0$, \eqref{eqn:Z_D_variational} recovers the term of optimal contribution from the RHS of \eqref{eqn:Z_D_innerproduct} and hence is a lower bound of $\calZ_D^\star$; secondly, \eqref{eqn:Z_D_variational} can be regarded as the saddle approximation to $\calZ_D^\star$ by picking up the term with maximal contribution.
\red{Interpreted as degenerated states.}


\begin{figure}[h]
  \centering
  \subfloat[Auxiliary Fine-Grained $\vec{S}_\gamma $-$ \vec{T}_\gamma$ Space.]{\includegraphics[width=0.48\textwidth]{auxilary_grid.png}
  \label{fig:1}}
  \hfill
  \subfloat[Cool Plot2.]{\includegraphics[width=0.48\textwidth]{auxilary_grid.png}
    \label{fig:2}}
  \caption{
  \hyperref[fig:1]{(a)} 
  We consider the case of $p=1$ for simplicity.
  The black grid and blue grid represent the $\vec{S}$-$\vec{T}$ and $\vec{S}_\gamma$-$\vec{T}_\gamma$ spaces, respectively.
  Each intersection of black (blue) dashed-line is a realization of $\vec{S}$-$ \vec{T}$ ($\vec{S}_\gamma$-$\vec{T}_\gamma$) space.
  For any ($\vec{S}_\gamma$-$\vec{T}_\gamma$)-realization $(\vec{S}_\gamma,\vec{T}_\gamma)$ (the blue circle), we can expand a $\calX_{\vec{S}_\gamma,\vec{T}_\gamma,\gamma}$ (green box) around it capturing enclosed  $(\vec{S},\vec{T})$'s (red circles) with \eqref{eqn:local_set}, and compute $\calZ_{D,\gamma}^\star$ with \eqref{eqn:Z_D_variational}.
  \hyperref[fig:2]{(b)}XXX
  }
\end{figure}


By Lemma~\ref{lemma:E_decomposed_bound}, we can construct $\abs{\ln \calZ_{D}-
\ln \calZ_{D,\gamma}^\star}$ by considering the following inequality
\begin{align}
\calZ^\star_{D,\gamma}e^{-8\norm{J}_F\gamma N\sqrt{p}} 
&\le 
\max_{\vec{S},\vec{T}}
\exp\left(-\sum_{\mu=1}^{p}S_{\mu}T_{\mu}
d_{\mu}\right)\left(\sum_{\{\bX:\Vec{S}(\bX)
=\Vec{S},\Vec{T}(\bX)=\Vec{T}\}}
1\)
\annot{(By Corollary~\ref{coro:exp_dst})}
\\
&\leq \calZ_{D} \label{eqn:Z_D_ineq1}
\\
&\leq
\sum_{\Vec{S}_\gamma,\Vec{T}_\gamma\in I_{\gamma}^{p}}\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}} 
\exp{-\sum_{\mu=1}^{p}S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)} d_{\mu}}\exp{8\norm{J}_F\gamma N\sqrt{p}}  
\annot{(By Corollary~\ref{coro:dst_parity} \& \ref{coro:exp_dst})}
\\
& \leq   
\( \sum_{\Vec{S}_\gamma,\Vec{T}_\gamma\in I_{\gamma}^{p} } 1\)
\calZ^\star_{D,\gamma}
\exp{8\norm{J}_F\gamma  N\sqrt{p}}
= 
\abs{I_{\gamma}}^{2p}
\calZ^\star_{D,\gamma}  \exp{8\norm{J}_F\gamma N\sqrt{p}},\label{eqn:Z_D_ineq2}
\end{align}
where $\abs{I_{\gamma}}^{2p}$ is the total number of \textit{all} possible configurations in $\vec{S}_\gamma$-$\vec{T}_\gamma$ space\footnote{$\abs{I_{\gamma}}^{2p}$ is not necessarily the same as $|\{\bX\}|$ because we do not consider the 1-1 identification map from $\bX$ to $(\vec{S}(\bX),\vec{T}(\bX))$ here, i.e. the
$\left(\sum_{\{\bX|\Vec{S}(\bX)=\Vec{S},\Vec{T}(\bX)=\Vec{T}\}}1\)$ term in \eqref{eqn:Z_D_innerproduct}.}.
Consequently, from \eqref{eqn:Z_D_ineq1} and \eqref{eqn:Z_D_ineq2} we get
\begin{equation}
\label{eqn:Z_D_upper}
\ln \calZ^\star_{D,\gamma}\leq\ln \calZ_{D}+8\norm{J}_F\gamma N\sqrt{p},
\end{equation}
and 
\begin{align}
\label{eqn:Z_D_lower}
\ln \calZ_{D,\gamma}^\star
&\geq\ln \calZ_{D}-8\norm{J}_F\gamma N\sqrt{p} - 2p\ln \abs{I_\gamma} \nonumber\\
&\ge \ln \calZ_{D}-8\norm{J}_F\gamma N\sqrt{p} - 2p\ln\(\frac{1}{\gamma} + 2\),
\end{align}
respectively.
These bounds allow us to control $\abs{\ln \calZ_{D}-\ln \calZ_{D,\gamma}^\star}$ by
\bea
\green{
\boxed{
\abs{\ln \calZ_{D}-\ln \calZ_{D,\gamma}^\star}
\le
8\norm{J}_F\gamma N\sqrt{p} + 2p\ln\(\frac{1}{\gamma} + 2\),
}
}
\label{eqn:bound3}
\eea
with variational parameter $\gamma\in(0,1)$ whose optimal value will be determined shortly.



We use and modify the results of \cite[Theorem~1]{jain2018mean}.
In order to construct bounds to control $\abs{\mathcal{F}^\star_D -\ln \calZ_{D,\gamma}^\star}$,
we need to develop mean-field description for $\ln \calZ_{D,\gamma}^\star$.

\green{
For any $\epsilon > 0$,
let $\gamma=\epsilon\sqrt{p}/48$.
}

We first write down the auxiliary Ising model defined by \eqref{eqn:Z_D_variational}
on $\vec{S}_{\gamma}$-$\vec{T}_\gamma$ as
\bea
\calZ_{D,\gamma}
\coloneqq
\sum_{\vec{S}_\gamma,\vec{T}_\gamma\in I_{\gamma}^{p}}\[\exp{-\sum_{\mu=1}^{p}S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)}d_{\mu}}
\bigg(\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}}\bigg)\]
,
\eea
and observe that the maximally contributed term \eqref{eqn:Z_D_variational}
is evaluated at a particular optimal realization $(\Vec{S}_\gamma, \Vec{T}_\gamma)$, 
and is restricted in a rather small configuration space defined by $\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}$.
That is, while \eqref{eqn:Z_D_variational} only has one configuration in $\vec{S}_\gamma$-$\vec{T}_\gamma$ space, it corresponds to multiple $\bX$'s captured by $\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}$ (the green box in Figure~\ref{fig:1}).

Naturally, for the optimal realization $(\vec{S}_\gamma,\vec{T}_\gamma)$,  \eqref{eqn:Z_D_variational} can be interpreted as the inner-product representation of a \textit{local} Ising model restricted by $\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}$. 
We define the corresponding auxiliary (naive) mean-field value, following \eqref{eqn:naive_MF},
\bea
\bar{y}_j \coloneqq \frac{1}{\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}}} \sum_{\bX \in \calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}} \bx_j,
\quad \(\;\bar{Y}\coloneqq \( \bar{y}_1,\cdots,\bar{y}_N\)\;\)
\eea
as the mean value of configurations captured by $\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}$.
Moreover, we denote probabilities associated to the \textit{restricted} configurations in $\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}$ for such a \textit{local} and \textit{restricted} Ising model as
$\bY \coloneqq (\by_1, \cdots, \by_N)\in [0,1]^N$.
As a result, 
the term 
$\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}}$ 
is nothing but the entropy $H(\bY)$ of the \textit{local} and \textit{restricted}  auxiliary Ising model $\calZ_D^\star$.
Therefore, we have
\begin{align}
\ln \abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}} &= H(\bY) \label{eqn:H_Y}
\\
&\le \sum_{j = 1}^N H(\by_j) 
= \sum_{j = 1}^N H\(\frac{1 + \overline{y}_j}{2}\),
\annot{(By \eqref{eqn:naive_MF})}
\end{align}
where the independent decomposition property of naive mean-field is used in the second line.







Taking logarithm of \eqref{eqn:Z_D_variational}, we have 
\begin{align}
\label{eqn:bound3.5}
\ln \calZ_{D,\gamma}^\star 
& =
-\sum_{\mu=1}^{p}S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)} d_{\mu}
+\ln\abs{\calX_{\Vec{S}_\gamma,\Vec{T}_\gamma,\gamma}}
\\
& \leq
-\sum_{\mu=1}^{p} S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)} d_{\mu}
+\sum_{j = 1}^N H\left(\frac{1 + \overline{y}_j}{2}\right)
\annot{(By \eqref{eqn:H_Y})}
\\
 & \leq
 \[-\sum_{\mu=1}^{p} S_{\mu}^{(\gamma)}T_{\mu}^{(\gamma)} d_{\mu}+8\norm{J}_F\gamma N \sqrt{p}
 \]
 +\sum_{j = 1}^N H\left(\frac{1 + \overline{y}_j}{2}\right)
 \annot{(By Lemma~\ref{lemma:E_decomposed_bound})}
\\
 & \leq
 \[ 
 \sum_{\mu=1}^{p}
 -S_{\mu}\(\bar{Y}\)T_{\mu}(\bar{Y})d_{\mu}+8\norm{J}_F\gamma N \sqrt{p}\] + \sum_{j = 1}^N H\left(\frac{1 + \overline{y}_j}{2}\right)
 \annot{(By Jensen's inequality)}
 \\
 & \leq -\mathcal{F}_{D}^\star+8\norm{J}_F\gamma N\sqrt{p}.
 \annot{(By \eqref{eqn:naive_MF})}
\end{align}
By combining \eqref{eqn:bound3} and \eqref{eqn:bound3.5}, we are able to control $\green{
\abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}
+\abs{\ln \calZ_{D,\gamma}^\star+\mathcal{F}^\star_D}
}$.
Firstly, one notice that
\begin{align} 
-\mathcal{F}_{D}^\star 
& \geq \ln \calZ_{D,\gamma}^\star - 8\norm{J}_F\gamma N\sqrt{p}\nonumber
\\
& \geq \ln \calZ_{D} - 16\norm{J}_F\gamma N\sqrt{p} - 2p\ln(\frac{1}{\gamma} + 2)
\annot{(By \eqref{eqn:Z_D_lower})}
\\
 & \geq \ln \calZ_{D} - \frac{\epsilon }{3}N\norm{J}_F - 9216\ln\left(\frac{48}{\epsilon} + \sqrt{2}\right)\frac{1}{\epsilon^{2}},
\end{align}
where in the last line,
for any $\epsilon > 0$,
 we choose $\gamma=\epsilon/(48\sqrt{p})$ and $p\le 2304/\epsilon^2$ in order to obtain the $\epsilon/3$ factor in front of the second term, and the inequality $(a+b)^2\le a^2+b^2$.
Secondly, by noticing $\mathcal{F}^\star_D + \ln \calZ_{D}\geq 0$,
we arrive 
\bea
0 \leq \ln \calZ_{D}+\mathcal{F}^\star_D \leq   \frac{\epsilon }{3}N\norm{J}_F + 9216\ln\left(\frac{48}{\epsilon} + \sqrt{2}\right)\frac{1}{\epsilon^{2}},
\eea
which implies
\bea
\label{eqn:bound4}
\green{
\boxed{
\abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}
+\abs{\ln \calZ_{D,\gamma}^\star+\mathcal{F}^\star_D}
\le 
\green{
\frac{\epsilon}{3}\epsilon n\norm{J}_F + 9216\ln\left(\frac{48}{\epsilon} + \sqrt{2}\right)\frac{1}{\epsilon^{2}}.
}
}}
\eea



\subsubsection{Step 3: Controlling $\abs{\calF^\star_{J,\text{naive}}-\mathcal{F}}$}
Combining above bounds \eqref{eqn:bound1&2}, \eqref{eqn:bound3} and \eqref{eqn:bound4}, for any $\epsilon > 0$, we get
\begin{align}
\calF^\star_{\text{naive}}-\mathcal{F}
&\leq  
\blue{
\abs{\ln \calZ -\ln\calZ_{D}}
}
+
\Blue{
\abs{\mathcal{F}^\star-\mathcal{F}^\star_{D}}
}
+
\green{
\abs{\ln \calZ_{D}- 
    \ln \calZ_{D,\gamma}^\star}
+\abs{\ln \calZ_{D,\gamma}^\star+\mathcal{F}^\star_D}
}
    \nonumber\\
& \le 
\blue{
\frac{\epsilon}{3} N \norm{J}_F
}+
\Blue{
\frac{\epsilon}{3} N \norm{J}_F 
}
+
\green{
\frac{\epsilon}{3} N \norm{J}_F + 9216\ln\left(\frac{48}{\epsilon} + \sqrt{2}\right)\frac{1}{\epsilon^{2}}
}
\nonumber\\
& \leq \epsilon N \norm{J}_F  + 9216\ln\left(\frac{48}{\epsilon} + \sqrt{2}\right)\frac{1}{\epsilon^{2}}<
\epsilon N \norm{J}_F  + 9216\ln\left(\frac{48}{\epsilon}+e\right)\frac{1}{\epsilon^{2}},
\label{eqn:bound5}
\end{align}
where we introduce $e$ in the last line to ensure $\ln(\cdot)\ge 1$. 

\begin{center}
    \red{Below Not Finished.}
\end{center}
Before getting technical, it is convenient to introduce some intuitions \red{that bound about $\(N\norm{J}_F\)^{2/3}$.}

In order to get the minimal dependence of $N\norm{J}_F,$ we let two competing terms be the same. Difference of absolute value of $\ln\(1/\epsilon\)$ is smaller than difference of absolute value $1/\epsilon^2$. One can verify it by computing their ratio of derivatives\footnote{$\lim_{\epsilon \to 0 } \nicefrac{\frac{\dd \(1/\epsilon^2\) }{\dd \epsilon }}{\frac{\dd \ln\(1/\epsilon\) }{\dd \epsilon }} =\lim_{\epsilon \to 0 }\nicefrac{2}{\epsilon^2}= \infty.$}. 
By letting two terms be the same and neglect the $\ln$ term, we have $\epsilon N\norm{J}_F \propto 1/\epsilon^2$.
We have $\epsilon \propto \(N \norm{J}_F\) ^{-1/3}$. If we plug $\epsilon$ back \eqref{eqn:bound5}, 
we find the bound is proportional to  $(N\norm{J}_F)^{2/3}$ modulo $\ln$ term. 
Below we will show that this is indeed the case for all $N\norm{J}_F.$  We also get the Intuition that in order to find optimal $\epsilon$ for $N\norm{J}_F$, we need to compare $\frac{1}{\epsilon}$ and $N\norm{J}_F$ magnitude.








{\color{blue}{We can finally achieve the result in terms of $N, \beta, ||J||_{F}.$}}



We need to choose the optimal $\epsilon$ to find tightest bound of  \eqref{eqn:bound5} where the two terms compete with each other. 
We need to discuss the following two cases:
\begin{itemize}
    \item 
    First we consider 
\bea \label{condi-1}
\frac{1}{\epsilon}<N \norm{J}_F,
\eea
with fixed a lower bound $M$ such that $M \geq e$ and $N\norm{J}_F>M.$ We then take $\epsilon = \left(\frac{M\ln(48 N \norm{J}_F + e)}{N \norm{J}_F \ln{M}}\right)^{1/3}.$ 
We notice the following trivial inequality: 
\bea \label{tri}
\frac{\ln M}{M} \leq 1 \leq N^2\norm{J}_F^2 \ln\(48 N\norm{J}_F+e\),
\eea
since $M>1$ and $\ln(48 N\norm{J}_F+e)>1$.
So we can check \eqref{condi-1}:
\bea
\frac{1}{\epsilon}
=N^{1/3}\norm{J}_F^{1/3} \(\frac{\ln M}{M \ln(48 N\norm{J}_F+e)}\)^{\nicefrac{1}{3}} \leq N \norm{J}_F
\eea
here we use \eqref{tri}.
We then have:
\bea
\ln\left(\frac{48}{\epsilon}+e\right) \leq  \ln\left(48 N \norm{J}_F+e\right)
\eea
So we have:
\bea
\calF^\star_{\text{naive}}-\mathcal{F} 
&\leq& \(\frac{M}{\ln M}\)^{\nicefrac{1}{3}} N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}\(48N \norm{J}_F + e\)\\  &&+ 9216\(\frac{\ln M}{M}\)^{\nicefrac{2}{3}} \frac{\ln(48 N \norm{J}_F + e)}{\ln^{\nicefrac{2}{3}}\(48 N \norm{J}_F + e\)} N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \nonumber \\
&\leq&
N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}\(48 N \norm{J}_F + e\)
\[\(\frac{M}{\ln M}\)^{\nicefrac{1}{3}} + 9216 \(\frac{\ln M}{M}\)^{\nicefrac{2}{3}}\].
\eea
Finally, taking $\(\frac{M}{\ln M}\) = 9216$, we find that $N \norm{J}_F$,
\bea
\mathcal{F}^*_{\text{naive}}- \mathcal{F}
\le 42 N^{\nicefrac{2}{3}} \norm{J}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}(48 N \norm{J}_F + e). 
\eea

    \item
    Now we can consider another case $N\norm{J}_F \leq M.$ From Lemma~\ref{lemma:trivial_bound_naiveMF},
    we have $\calF^\star_{\text{naive}}-\mathcal{F} \leq N\norm{J}_F$. 
    Therefore, if $N \norm{J}_F \leq M$, we see that $\calF^\star_{\text{naive}}-\mathcal{F} \le N \norm{J}_F \leq M^{\nicefrac{1}{3}} (N \norm{J}_F)^{\nicefrac{2}{3}}$.
\end{itemize}

We then combine two cases and show that for all $N \norm{J}_F$ and then restore all coefficients. So we have: 
\bea
\boxed{
\calF^\star_{RNN}-\mathcal{F}\leq 
\calF^\star_{\text{naive}}-\mathcal{F} \leq \frac{1}{\beta} \calO\(N^{\nicefrac{2}{3}} \norm{\beta \tilde{ J}}_F^{\nicefrac{2}{3}} \ln^{\nicefrac{1}{3}}\(N \norm{\beta \tilde{J}}_F\)\)
}
\eea
which leads to our final bound. 
\end{proof}




\clearpage

































    

    
    






    
    
    





